PAPER: Privacy-Preserving Convolutional Neural Networks using Low-Degree Polynomial Approximations and Structural Optimizations on Leveled FHE

Recent work using Fully Homomorphic Encryption (FHE) has made non-interactive privacy-preserving inference of deep Convolutional Neural Networks (CNNs) possible. However, the performance of these methods remains limited by their heavy reliance on bootstrapping, a costly FHE operation applied across multiple layers that severely slows inference. Moreover, they depend on high-degree polynomial approximations of non-linear activations, which increase multiplicative depth and reduce accuracy by 2-5% compared with plaintext ReLU models. In this work, we close the accuracy gap between FHE-based non-interactive CNNs and their plaintext counterparts while achieving faster inference than existing methods. We propose a quadratic polynomial approximation of ReLU that achieves the theoretical minimum multiplicative depth for non-linear activations, together with a penalty-based training strategy. We further introduce structural optimizations that reduce the required FHE levels in CNNs by a factor of five compared with prior work, allowing us to run deep CNN models under leveled FHE without bootstrapping. To further accelerate inference and recover accuracy typically lost with polynomial approximations, we introduce parameter clustering together with a joint strategy involving data layout and ensemble techniques. Experiments with VGG and ResNet models on CIFAR and Tiny-ImageNet datasets show that our approach achieves up to 4x faster private inference than prior work, with accuracy comparable to plaintext ReLU models.

==> tables/resnet18.tex <==
\begin{table*}[!t]
    \centering
    \small
    \caption
    {
        Accuracy, inference time, and peak memory for CIFAR-10 and CIFAR-100 on ResNet-18.
    }
    \begin{tabular}
    {
        C{0.6cm} |
        C{0.7cm} |
        C{0.7cm} |
        C{0.6cm} |
        C{0.6cm} |
        C{1.0cm} 
        C{0.0cm} 
        C{0.6cm} |
        C{0.7cm} |
        C{0.7cm} |
        C{0.6cm} |
        C{0.6cm} | 
        C{1.0cm}
    }

        % Standard
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Standard} & {} & \multicolumn{6}{c}{Standard} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{M} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{M} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        1 & 93.73 & 0.27 & 3925 & 51 & 292 & {} & 1 & 74.96 & 0.51 & 3935 & 79 & 338 \\
        2 & 94.34 & 0.16 & 3930 & 54 & 314 & {} & 2 & 76.48 & 0.28 & 3874 & 40 & 355 \\
        4 & 94.69 & 0.12 & 3840 & 44 & 347 & {} & 4 & 77.43 & 0.24 & 3929 & 54 & 390 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Full Clustering (M = 1)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Full Clustering (M = 1)} & {} & \multicolumn{6}{c}{Full Clustering (M = 1)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        2 & 10.16 & 0.72 & 404 & 16 & 187 & {} & 2 & 1.00 & 0.07 & 414 & 25 & 229 \\
        4 & 10.14 & 0.89 & 406 & 18 & 187 & {} & 4 & 1.02 & 0.12 & 413 & 17 & 228 \\
        8 & 9.91 & 1.48 & 420 & 31 & 187 & {} & 8 & 1.08 & 0.17 & 426 & 23 & 229 \\
        16 & 15.89 & 7.51 & 427 & 27 & 188 & {} & 16 & 2.01 & 1.10 & 430 & 25 & 228 \\
        32 & 70.18 & 14.19 & 439 & 28 & 188 & {} & 32 & 32.33 & 13.66 & 441 & 23 & 228 \\
        64 & 91.42 & 1.25 & 481 & 31 & 188 & {} & 64 & 68.01 & 4.00 & 484 & 34 & 229 \\
        128 & 93.24 & 0.29 & 530 & 34 & 188 & {} & 128 & 72.62 & 1.04 & 554 & 41 & 228 \\
        256 & 93.53 & 0.26 & 619 & 36 & 189 & {} & 256 & 73.98 & 0.68 & 646 & 44 & 230 \\
        512 & 93.65 & 0.25 & 719 & 40 & 189 & {} & 512 & 74.50 & 0.70 & 773 & 53 & 230 \\
        1024 & 93.69 & 0.28 & 856 & 34 & 196 & {} & 1024 & 74.65 & 0.69 & 926 & 58 & 237 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 1)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 1)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 1)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        2 & 9.79 & 0.76 & 418 & 32 & 188 & {} & 2 & 1.07 & 0.17 & 426 & 16 & 228 \\
        4 & 12.66 & 3.02 & 409 & 23 & 187 & {} & 4 & 2.76 & 1.17 & 413 & 13 & 229 \\
        8 & 81.28 & 6.04 & 412 & 23 & 187 & {} & 8 & 42.21 & 13.71 & 420 & 24 & 230 \\
        16 & 92.25 & 0.68 & 420 & 19 & 188 & {} & 16 & 69.28 & 2.37 & 443 & 25 & 228 \\
        32 & 93.36 & 0.33 & 456 & 28 & 188 & {} & 32 & 72.85 & 0.92 & 466 & 27 & 229 \\
        64 & 93.62 & 0.27 & 504 & 30 & 188 & {} & 64 & 74.31 & 0.77 & 520 & 31 & 229 \\
        128 & 93.70 & 0.26 & 586 & 30 & 189 & {} & 128 & 74.61 & 0.73 & 602 & 36 & 229 \\
        256 & 93.70 & 0.28 & 696 & 34 & 189 & {} & 256 & 74.68 & 0.71 & 724 & 39 & 230 \\
        512 & 93.73 & 0.27 & 855 & 58 & 192 & {} & 512 & 74.69 & 0.73 & 874 & 49 & 235 \\
        1024 & 93.72 & 0.27 & 1016 & 57 & 203 & {} & 1024 & 74.71 & 0.74 & 1066 & 66 & 244 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 2)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 2)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 2)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        64 & 92.59 & 0.45 & 520 & 43 & 205 & {} & 64 & 68.93 & 1.94 & 524 & 10 & 247 \\
        128 & 93.85 & 0.15 & 597 & 38 & 206 & {} & 128 & 74.47 & 0.59 & 622 & 23 & 247 \\
        256 & 94.35 & 0.10 & 695 & 22 & 206 & {} & 256 & 75.79 & 0.43 & 734 & 51 & 247 \\
        512 & 94.50 & 0.09 & 854 & 28 & 210 & {} & 512 & 76.35 & 0.18 & 871 & 37 & 251 \\
        1024 & 94.60 & 0.08 & 1045 & 61 & 220 & {} & 1024 & 76.67 & 0.12 & 1049 & 23 & 261 \\
        2048 & 94.73 & 0.07 & 1164 & 36 & 240 & {} & 2048 & 76.82 & 0.14 & 1202 & 72 & 281 \\
        4096 & 94.78 & 0.04 & 1268 & 42 & 301 & {} & 4096 & 76.90 & 0.08 & 1308 & 18 & 342 \\
        8192 & 94.77 & 0.05 & 1482 & 59 & 459 & {} & 8192 & 76.97 & 0.07 & 1440 & 13 & 500 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 4)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 4)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 4)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        64 & 18.38 & 4.80 & 526 & 27 & 240 & {} & 64 & 1.73 & 0.41 & 538 & 26 & 281 \\
        128 & 35.79 & 8.02 & 621 & 45 & 240 & {} & 128 & 5.31 & 0.94 & 615 & 27 & 281 \\
        256 & 66.88 & 5.19 & 728 & 51 & 241 & {} & 256 & 29.69 & 2.16 & 750 & 47 & 282 \\
        512 & 84.28 & 2.38 & 866 & 28 & 245 & {} & 512 & 57.88 & 2.20 & 885 & 16 & 286 \\
        1024 & 91.47 & 0.46 & 1035 & 69 & 255 & {} & 1024 & 68.98 & 1.13 & 1057 & 46 & 297 \\
        2048 & 93.10 & 0.21 & 1211 & 57 & 275 & {} & 2048 & 73.96 & 0.38 & 1195 & 64 & 316 \\
        4096 & 94.11 & 0.14 & 1298 & 17 & 337 & {} & 4096 & 75.93 & 0.22 & 1263 & 24 & 378 \\
        8192 & 94.55 & 0.11 & 1509 & 22 & 494 & {} & 8192 & 76.66 & 0.12 & 1355 & 17 & 535 \\
        \cline{1-6} \cline{8-13}
    \end{tabular}
    \label{tab:resnet18}
\end{table*}

==> tables/resnet20.tex <==
\begin{table*}[!t]
    \centering
    \small
    \caption
    {
        Accuracy, inference time, and peak memory for CIFAR-10 and CIFAR-100 on ResNet-20.
    }
    \begin{tabular}
    {
        C{0.6cm} |
        C{0.7cm} |
        C{0.7cm} |
        C{0.6cm} |
        C{0.6cm} |
        C{1.0cm} 
        C{0.0cm} 
        C{0.6cm} |
        C{0.7cm} |
        C{0.7cm} |
        C{0.6cm} |
        C{0.6cm} | 
        C{1.0cm}
    }

        % Standard
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Standard} & {} & \multicolumn{6}{c}{Standard} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{M} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{M} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        1 & 94.06 & 0.26 & 1886 & 30 & 279 & {} & 1 & 73.89 & 0.37 & 1902 & 26 & 305 \\
        2 & 94.71 & 0.11 & 1884 & 41 & 300 & {} & 2 & 76.59 & 0.25 & 1874 & 27 & 320 \\
        4 & 95.04 & 0.10 & 1886 & 32 & 330 & {} & 4 & 77.97 & 0.13 & 1904 & 30 & 351 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Full Clustering (M = 1)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Full Clustering (M = 1)} & {} & \multicolumn{6}{c}{Full Clustering (M = 1)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        2 & 10.08 & 0.26 & 242 & 10 & 172 & {} & 2 & 1.03 & 0.07 & 246 & 6 & 192 \\
        4 & 10.08 & 0.32 & 246 & 6 & 172 & {} & 4 & 1.08 & 0.23 & 246 & 9 & 192 \\
        8 & 10.17 & 0.89 & 250 & 12 & 172 & {} & 8 & 1.17 & 0.24 & 252 & 7 & 192 \\
        16 & 14.44 & 6.34 & 260 & 13 & 172 & {} & 16 & 2.05 & 1.58 & 258 & 8 & 192 \\
        32 & 78.18 & 8.99 & 264 & 7 & 172 & {} & 32 & 32.59 & 14.07 & 272 & 16 & 192 \\
        64 & 92.46 & 0.95 & 288 & 10 & 172 & {} & 64 & 68.18 & 3.24 & 290 & 11 & 192 \\
        128 & 93.77 & 0.37 & 334 & 12 & 172 & {} & 128 & 71.56 & 1.19 & 334 & 15 & 192 \\
        256 & 94.00 & 0.26 & 407 & 22 & 172 & {} & 256 & 73.39 & 0.49 & 392 & 9 & 192 \\
        512 & 94.02 & 0.26 & 475 & 18 & 173 & {} & 512 & 73.75 & 0.35 & 473 & 20 & 193 \\
        1024 & 94.05 & 0.26 & 553 & 25 & 181 & {} & 1024 & 73.85 & 0.35 & 563 & 28 & 201 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 1)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 1)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 1)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        2 & 10.05 & 0.41 & 249 & 18 & 172 & {} & 2 & 1.12 & 0.22 & 254 & 10 & 192 \\
        4 & 14.59 & 4.33 & 244 & 7 & 172 & {} & 4 & 2.11 & 0.62 & 255 & 13 & 192 \\
        8 & 85.17 & 2.66 & 247 & 7 & 172 & {} & 8 & 49.94 & 5.99 & 264 & 21 & 192 \\
        16 & 93.20 & 0.45 & 262 & 6 & 172 & {} & 16 & 69.60 & 1.71 & 262 & 7 & 192 \\
        32 & 93.87 & 0.32 & 276 & 9 & 172 & {} & 32 & 72.98 & 0.45 & 292 & 12 & 192 \\
        64 & 94.01 & 0.28 & 314 & 9 & 172 & {} & 64 & 73.68 & 0.38 & 323 & 13 & 192 \\
        128 & 94.01 & 0.28 & 366 & 14 & 172 & {} & 128 & 73.85 & 0.38 & 377 & 18 & 192 \\
        256 & 94.04 & 0.27 & 442 & 10 & 172 & {} & 256 & 73.89 & 0.34 & 452 & 17 & 193 \\
        512 & 94.05 & 0.26 & 536 & 26 & 177 & {} & 512 & 73.89 & 0.36 & 538 & 10 & 198 \\
        1024 & 94.05 & 0.26 & 612 & 19 & 190 & {} & 1024 & 73.88 & 0.36 & 626 & 21 & 209 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 2)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 2)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 2)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        64 & 92.52 & 0.56 & 312 & 9 & 187 & {} & 64 & 68.98 & 0.97 & 321 & 14 & 208 \\
        128 & 94.34 & 0.10 & 370 & 8 & 187 & {} & 128 & 74.31 & 0.44 & 380 & 16 & 207 \\
        256 & 94.81 & 0.08 & 443 & 20 & 188 & {} & 256 & 76.08 & 0.25 & 464 & 7 & 208 \\
        512 & 94.93 & 0.08 & 531 & 31 & 192 & {} & 512 & 76.65 & 0.19 & 541 & 22 & 213 \\
        1024 & 95.08 & 0.07 & 611 & 14 & 205 & {} & 1024 & 76.99 & 0.11 & 614 & 22 & 226 \\
        2048 & 95.11 & 0.06 & 679 & 7 & 239 & {} & 2048 & 77.16 & 0.13 & 690 & 23 & 259 \\
        4096 & 95.08 & 0.04 & 814 & 60 & 333 & {} & 4096 & 77.12 & 0.12 & 746 & 17 & 354 \\
        8192 & 95.08 & 0.03 & 885 & 37 & 541 & {} & 8192 & 77.23 & 0.09 & 897 & 26 & 556 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 4)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 4)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 4)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        64 & 12.79 & 2.88 & 332 & 14 & 219 & {} & 64 & 1.72 & 0.48 & 341 & 13 & 240 \\
        128 & 25.95 & 4.81 & 389 & 7 & 219 & {} & 128 & 3.86 & 0.96 & 407 & 10 & 239 \\
        256 & 57.23 & 3.93 & 455 & 21 & 219 & {} & 256 & 19.97 & 2.42 & 463 & 19 & 239 \\
        512 & 83.18 & 1.59 & 534 & 10 & 224 & {} & 512 & 52.26 & 2.81 & 546 & 8 & 244 \\
        1024 & 91.45 & 0.46 & 603 & 18 & 237 & {} & 1024 & 68.37 & 0.63 & 631 & 14 & 256 \\
        2048 & 93.89 & 0.26 & 648 & 9 & 270 & {} & 2048 & 73.73 & 0.53 & 673 & 11 & 290 \\
        4096 & 94.65 & 0.16 & 722 & 12 & 365 & {} & 4096 & 76.44 & 0.31 & 765 & 9 & 386 \\
        8192 & 94.90 & 0.10 & 815 & 17 & 571 & {} & 8192 & 77.62 & 0.17 & 855 & 16 & 588 \\
        \cline{1-6} \cline{8-13}
    \end{tabular}
    \label{tab:resnet20}
\end{table*}

==> tables/resnet32.tex <==
\begin{table*}[!t]
    \centering
    \small
    \caption
    {
        Accuracy, inference time, and peak memory for CIFAR-10 and CIFAR-100 on ResNet-32.
    }
    \begin{tabular}
    {
        C{0.6cm} |
        C{0.7cm} |
        C{0.7cm} |
        C{0.6cm} |
        C{0.6cm} |
        C{1.0cm} 
        C{0.0cm} 
        C{0.6cm} |
        C{0.7cm} |
        C{0.7cm} |
        C{0.6cm} |
        C{0.6cm} | 
        C{1.0cm}
    }

        % Standard
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Standard} & {} & \multicolumn{6}{c}{Standard} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{M} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{M} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        1 & 93.86 & 0.24 & 9405 & 109 & 1332 & {} & 1 & 73.93 & 0.53 & 8865 & 132 & 1401 \\
        2 & 94.69 & 0.18 & 8854 & 80 & 1394 & {} & 2 & 76.79 & 0.34 & 8902 & 152 & 1418 \\
        4 & 94.99 & 0.13 & 8813 & 63 & 1441 & {} & 4 & 78.34 & 0.23 & 8907 & 141 & 1465 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Full Clustering (M = 1)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Full Clustering (M = 1)} & {} & \multicolumn{6}{c}{Full Clustering (M = 1)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        2 & 10.12 & 0.22 & 1578 & 63 & 794 & {} & 2 & 0.98 & 0.07 & 1544 & 5 & 836 \\
        4 & 10.13 & 0.21 & 1538 & 3 & 795 & {} & 4 & 0.98 & 0.07 & 1577 & 20 & 836 \\
        8 & 10.12 & 0.22 & 1588 & 79 & 794 & {} & 8 & 0.97 & 0.07 & 1540 & 24 & 836 \\
        16 & 10.35 & 1.35 & 1570 & 8 & 795 & {} & 16 & 1.03 & 0.21 & 1547 & 27 & 837 \\
        32 & 37.13 & 16.87 & 1578 & 3 & 795 & {} & 32 & 3.91 & 2.63 & 1565 & 13 & 836 \\
        64 & 86.61 & 3.69 & 1703 & 80 & 795 & {} & 64 & 52.92 & 7.49 & 1686 & 44 & 837 \\
        128 & 92.82 & 0.47 & 2131 & 27 & 794 & {} & 128 & 70.26 & 1.24 & 1819 & 5 & 836 \\
        256 & 93.70 & 0.32 & 2164 & 151 & 795 & {} & 256 & 73.18 & 0.38 & 2013 & 33 & 837 \\
        512 & 93.84 & 0.27 & 2495 & 164 & 796 & {} & 512 & 73.75 & 0.37 & 2381 & 70 & 837 \\
        1024 & 93.86 & 0.26 & 2898 & 174 & 837 & {} & 1024 & 73.89 & 0.33 & 2822 & 53 & 871 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 1)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 1)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 1)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        2 & 10.12 & 1.07 & 1605 & 57 & 795 & {} & 2 & 0.99 & 0.08 & 1559 & 11 & 836 \\
        4 & 10.00 & 0.99 & 1573 & 24 & 795 & {} & 4 & 1.00 & 0.09 & 1526 & 27 & 836 \\
        8 & 34.61 & 12.19 & 1601 & 65 & 795 & {} & 8 & 9.67 & 5.64 & 1586 & 11 & 837 \\
        16 & 89.08 & 2.44 & 1559 & 6 & 795 & {} & 16 & 60.50 & 4.61 & 1576 & 8 & 837 \\
        32 & 93.12 & 0.49 & 1761 & 90 & 795 & {} & 32 & 71.75 & 0.80 & 1679 & 19 & 836 \\
        64 & 93.75 & 0.29 & 1833 & 54 & 795 & {} & 64 & 73.49 & 0.36 & 1803 & 9 & 836 \\
        128 & 93.84 & 0.26 & 2077 & 111 & 794 & {} & 128 & 73.83 & 0.33 & 2027 & 30 & 836 \\
        256 & 93.86 & 0.27 & 2488 & 185 & 796 & {} & 256 & 73.91 & 0.33 & 2379 & 83 & 838 \\
        512 & 93.85 & 0.25 & 2849 & 128 & 818 & {} & 512 & 73.93 & 0.33 & 2815 & 60 & 860 \\
        1024 & 93.86 & 0.24 & 3317 & 192 & 883 & {} & 1024 & 73.94 & 0.53 & 3313 & 57 & 925 \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 2)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 2)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 2)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        64 & 85.12 & 4.61 & 1831 & 69 & 820 & {} & 64 & 52.29 & 6.60 & 1791 & 17 & 861 \\
        128 & 92.75 & 0.58 & 2069 & 79 & 820 & {} & 128 & 70.20 & 1.26 & 2014 & 44 & 861 \\
        256 & 94.06 & 0.21 & 2388 & 156 & 821 & {} & 256 & 74.51 & 0.42 & 2340 & 52 & 862 \\
        512 & 94.59 & 0.12 & 2788 & 167 & 843 & {} & 512 & 76.30 & 0.25 & 2809 & 38 & 884 \\
        1024 & 94.76 & 0.12 & 3093 & 11 & 908 & {} & 1024 & 76.77 & 0.24 & 3238 & 64 & 951 \\
        2048 & 94.86 & 0.06 & 3602 & 32 & 1083 & {} & 2048 & 77.24 & 0.08 & 3797 & 64 & 1125 \\
        4096 & 94.95 & 0.07 & 4043 & 59 & 1573 & {} & 4096 & 77.33 & 0.07 & 4388 & 28 & 1615 \\
        % 8192 & 94.90 & 0.05 & \multicolumn{3}{c}{out of memory} & {} & 8192 & 77.31 & 0.08 & \multicolumn{3}{c}{out of memory} \\
        \cline{1-6} \cline{8-13}
        \multicolumn{13}{c}{} \\

        % Slice Clustering (M = 4)
        \cline{1-6} \cline{8-13}
        
        \multicolumn{6}{c}{Slice Clustering (M = 4)} & {} & \multicolumn{6}{c}{Slice Clustering (M = 4)} \\
        \cline{1-6} \cline{8-13}

        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} & {} &
        \multirow{2}*{k} &
        \multicolumn{2}{c|}{Accuracy (\%)} &
        \multicolumn{2}{c|}{Inf. Time (s)} &
        {Memory} \\

        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} & {} &
        {} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & \multicolumn{1}{c}{\it $\mu$} & {\it $\sigma$} & {(GB)} \\  
        \cline{1-6} \cline{8-13} 

        64 & 9.27 & 0.65 & 1845 & 89 & 870 & {} & 64 & 0.92 & 0.00 & 1817 & 22 & 912 \\
        128 & 14.20 & 2.55 & 2096 & 100 & 870 & {} & 128 & 0.92 & 0.01 & 2031 & 26 & 911 \\
        256 & 30.01 & 9.08 & 2409 & 149 & 871 & {} & 256 & 1.79 & 0.74 & 2367 & 50 & 912 \\
        512 & 69.18 & 5.72 & 2842 & 193 & 894 & {} & 512 & 16.68 & 6.66 & 2823 & 47 & 935 \\
        1024 & 88.24 & 1.02 & 3379 & 64 & 958 & {} & 1024 & 47.96 & 5.14 & 3495 & 15 & 1001 \\
        2048 & 92.32 & 0.68 & 3657 & 123 & 1133 & {} & 2048 & 65.54 & 1.33 & 3740 & 59 & 1175 \\
        4096 & 94.14 & 0.24 & 4301 & 130 & 1624 & {} & 4096 & 73.88 & 0.63 & 4199 & 60 & 1664 \\
        % 8192 & 94.89 & 0.16 & \multicolumn{3}{c}{out of memory} & {} & 8192 & 76.89 & 0.23 & \multicolumn{3}{c}{out of memory} \\
        \cline{1-6} \cline{8-13}
    \end{tabular}
    \label{tab:resnet32}
    \vspace{0.7cm}
\end{table*}
